IPv6 over Bluetooth Advertisements: An alternative approach to IP over BLE

The IPv6 over Bluetooth Low Energy (BLE) standard defines the transfer of IP data via BLE connections. This connection-oriented approach provides high reliability but increases packet delays and requires substantial overhead to manage BLE connections. To overcome these drawbacks we present the design and implementation of IPv6 over BLE advertisements, a standard-compliant connection-less approach. We deploy our proposal on low-power IoT hardware and comparatively measure key network performance metrics in a public testbed. Our results show that IP over BLE advertisements offers network performance characteristics complementary to IP over connection-based BLE, trading lower reliability for shorter~latency.

==> sections/acks.tex <==
%!TEX root = ../main.tex

\subsection*{Acknowledgments}
We would like to thank the anonymous reviewers and our shepherd TBD for their valuable feedback.
This work was supported in parts by the German Federal Ministry of Education and Research (BMBF) within the 5G project \emph{I3} and the VIP+ project \emph{RAPstore}.


